MONAL: Model Autophagy Analysis for Modeling Human-AI Interactions

The increasing significance of large models and their multi-modal variants in societal information processing has ignited debates on social safety and ethics. However, there exists a paucity of comprehensive analysis for: (i) the interactions between human and artificial intelligence systems, and (ii) understanding and addressing the associated limitations. To bridge this gap, we propose Model Autophagy Analysis (MONAL) for large models' self-consumption explanation. MONAL employs two distinct autophagous loops (referred to as ``self-consumption loops'') to elucidate the suppression of human-generated information in the exchange between human and AI systems. Through comprehensive experiments on diverse datasets, we evaluate the capacities of generated models as both creators and disseminators of information. Our key findings reveal (i) A progressive prevalence of model-generated synthetic information over time within training datasets compared to human-generated information; (ii) The discernible tendency of large models, when acting as information transmitters across multiple iterations, to selectively modify or prioritize specific contents; and (iii) The potential for a reduction in the diversity of socially or human-generated information, leading to bottlenecks in the performance enhancement of large models and confining them to local optima.

==> 3b_analyses.tex <==

\subsection{Analyses}
\label{sec:Analyses}

\subsubsection{Information Selection Biases\eat{ in Human and Language Model Interactions}}

\noindent {\bf LLMs can identify the quality of response as 
information filters but are obviously biased towards synthetic data.
\fixshu{FIXED check it}} 

Table~\ref{table:exp1} displays the cross-scoring results for various 
LLMs on a scale (0-5). 
These results help us understand that
LLMs do have an inherent capability to comprehend 
specific criteria in Table~\ref{appendix:Cross_scoring_Prompt} 
and can adjust the quality of their generated answers based 
on relevant instructions. 

However, when scoring data according to these 
criteria, each model exhibits certain preferences.

Specifically, models tend to assign higher scores to the high-quality 
answers generated by themselves, particularly for ChatGPT and GPT-4, 
which both demonstrate high confidence in their own outputs. 
Also, we find that 
ChatGPT and GPT-4 exhibit similar characteristics in scoring; 
they are inclined to extreme scores, i.e., high or low scores 
(assigning scores of 1 or 5 with very high probability), 
at the same time, they both tend to 
assign lower scores to Claude2 and PaLM 2 chat-bison.
These results are aligned with earlier research by~
\citet{liu2023llms} that emphasized that current 
top-performing LLMs (both black-box and white-box)
are narcissistic evaluators.\fixme{Move text to concluding results}


While evaluating the abilities of LLMs as 
\warn{answer generators\eat{of answers}}, ChatGPT’s worst 
quality answers can still deceptively obtain higher scores 
from other models, that are easy to figure out for humans 
via crowd-sourcing.
\eat{ workers can tell them.} 
\eat{At the same time, as the generator of answers, ChatGPT’s worst quality 
answers can still deceptively obtain higher scores from other models, 
but human crowd-sourcing workers can tell them.}
Furthermore, we observed that Claud2 tends to favor neutral 
and 'less controversial' ratings, often 
assigning average scores, i.e., 3 or 4, even for the worst quality answers. 
This is also reflected by a relatively higher score assigned 
by Claud2 to low-quality answers compared to other models. 
\eat{is much higher than that of other models,} 
Also, the difference between its score for initial answers and 
best-quality answers is not significant.


Llama-2-70b-chat and Solar-0-70B-16bit show similar scoring and generation behaviors, which may be attributable to the fact
that \warn{Solar-0-70B-16bit is fine-tuned form LLaMA-2-70b with only Orca-style and 
Alpaca-style dataset,
\fixshu{FIXED fine-tuned using LLAma-2-70B instructions..?}
indicating that the pre-trained model has a significant influence on the model's preferences.}

We observed that prompting the model to generate better answers did 
not always lead to higher scores in our experiments. Only Claud2 
showed significant improvement in the answers compared to the 
original responses. 
\warn{Conversely, when we prompt model generate poorer answers, the quality of answers generated by almost all LLMs in Table~\ref{table:exp1} decreased significantly. }
\fixshu{Fixed Re-write this line is not clear..!}

However, ChatGPT and Palm-2-chat-bision still achieved relatively high scores, a possible reason is could be attributed to the models being highly aligned to avoid producing harmful outputs~\cite{lambert2022illustrating}, so \warn{no matter what prompts we give them, they will try to give an answer that positively answers the question.}. 
\fixshu{FIXED How this alignment helps in achieving higher score..?}
We leave further investigation to our future work.

\fixshu{For this part, the heading says:\\
\textbf{LLMs can identify the quality of response as
information filters but are obviously biased
against real human data.} 
I think The true message is not conveyed as there is hardly any
discussion on real human data..????}

\warn{These facts remind us more cost-effective model training processes and wider applications are inevitable trends of large model development, so we need to discuss not only the technology of large models themselves but also the roles they play in their iterations and the development of human society \citep{tomavsev2020ai}.}\fixme{Asif move text}


\noindent {\bf Human-generated answers receive lower scores.} 
In Table \ref{table:exp1}, 
\fixshu{which part of Table~\ref{table:exp1}..?}
we observe that human-generated responses received relatively 
lower scores from the LLMs. 

Upon analysis, we found that human evaluators were able to objectively assess the answers produced by the LLMs, demonstrated by the fact that their scores for high-quality answers consistently remained above 4.00 when confronted with the results generated by the large language model, while the results for lower-quality answers remained below 3.00. 
\fixshu{Cut down the above sentence into two meaningful sentences.}

Furthermore, the scoring behavior of \eat{our 50 }crowd-sourced annotators toward the answers generated by the large language model was largely consistent. This may be due to the highly structured and standardized nature of answers produced by AI systems aligned with human feedback\eat{, which often received higher scores}. 
\warn{In contrast, human-generated answers received lower scores 
from the \fixshu{human..?} annotators, with significant variations 
among different evaluators. 
This may be attributed to the higher alignment degree between 
the large model and the human collective, compared to the 
alignment among individual humans.}
\fixshu{You mean humans are more aligned with LLMs,
compared to alignment between humans only.?}







\subsubsection{LLMs-generated Answers are more likely to Win in Information Screening}

To mitigate the impact of scoring criteria
\fixshu{what do yo mean by scoring criteria}
and excessive context length
\fixshu{why we need to mention excessive context length.?}
on the evaluative capabilities of large models and 
human evaluators, we simulated an examination grading scenario. 

For this, we used LLMs (ChatGPT, Claud2) and humans to simultaneously act as generators and evaluators.
The results for this experiment (Table \ref{table:Exam_Scenario_Simulation})
show that human answers were \warn{rarely} chosen as 
the best response, indicating a challenge in integrating authentic human-generated responses into the training data for models and the real-world human feedback loop.
\fixshu{say little more based on Table~\ref{table:Exam_Scenario_Simulation}.}
This finding substantiates the potential risks highlighted in Section \ref{sec:rat_risk} that
emphasized that human-generated responses receive comparatively lower scores.
\fixme{Asif: Correlate with Sec~\ref{sec:rat_risk}.}


\eat{Furthermore, we engaged ChatGPT, Claud2, and crowd annotators to select the best answers.}



\subsubsection{\eat{LLMs as Biased }Information Transmitters}
\input{tables/SDXL_0}
\input{tables/aiwashresult_img}
\eat{\noindent {\bf Large models exhibit inherent biases regarding the manner and content of conveyed information.}}

\noindent {\bf Large models are inherently biased.}
We claim that the large models are inherently biased 
regarding the manner and content of conveyed information.

\warn{For this, we...!\\
Where details + specs for AI-Washing experiments}.?

An example in this regard is illustrated in 
Table~\ref{table:aiwashtext}, where we show the 
results of a sample text data being refined simultaneously by ChatGPT five times.
We observe the refinements induced subtle shifts 
in the sample's language style and narrative technique.


We also repeat these experiments for the image data 
sets. For this, we used \textbf{\warn{SDXL}}\fixshu{FIXED add details} model to refine a set of images for 20 rounds. 
Corresponding results for a vast variety of images 
are shown in Figure~\ref{fig:SDXL_0.png} and \ref{fig:aiwashimag}.
These results \eat{show Our observations }reveal that repeatedly processing images with generative models is akin to information and feature filtration process. 
The model decides which specific aspects to preserve, diminish, or amplify \eat{based on its inherent \warn{biases.}
\fixshu{which biases.?}}

Specifically, in Figure \ref{fig:SDXL_0.png}, the 
model preserved the color distribution of the original
image but altered the main subject from a cat to a 
human portrait. 
Conversely, for the images in Figure~\ref{fig:aiwashimag}, 
we observed, a dominant alteration in image style rather than a change in the primary content for first, forth and fifth images.
Whereas, the images at second and third position underwent several iterations with minimal transformation, with the 
third image lost readability for the textual content.


This inconsistency may be attributed to the fact that while SDXL is renowned for generating high-quality images, the definition of quality in the context of generative models is subjective and heavily influenced by the annotations of the training dataset, also explained in detail by~\citet{podell2023sdxl}. 

These observations also indicate a bias in the model's processing, where certain features are selectively preserved or altered based on the model's training objective and inherent design. 
This in turn results in a higher probability of generating images containing specific features and/or information, e.g.,
loop, such as hand-drawn styles, portraits, close-ups of objects with clear backgrounds, etc.
To summarize, these findings demonstrate that large models are inherently biased regarding the manner and content of conveyed information.

% \input{tables/embedding0-4}


\noindent {\bf \eat{The risk to the fairness and }
Diversity of information spread.}

In order to further understand the training behaviour of large
models, we analyzed the cosine similarity scores during model 
training for humanly-generated and LLM-generated text.

\warn{The results in Figure~\ref{fig:average_simchange} shows that after processing text using LLMs, the similarity between texts significantly increases, with the lower similarity tail (showed as the $N = 1$ line with the Cosine similarity between 0.5 and 0.7) being 'washed out'.}
\fixshu{Re-write to make it explicit.}
\warn{This shows that \eat{We observe that }while acting as 
information disseminators, the large models exhibit some 
unique characteristics, i.e.,\eat{Their optimization objective} 
they tends to optimize more for real-world data while being 
more lenient towards self-generated samples.}
\eat{
To validate these findings, we perform a simple 
For this Experiments demonstrate that when}

% \input{tables/average_distributionchange}
% \input{tables/distributionresult}


Analyzing the model behavior across multiple runs, 
we can see that after approximately three iterations 
($N\approx3$), the difference in the average 
cosine similarity across multiple runs round tends 
to stabilize (Figure~\ref{fig:average_distributionchange}).
\warn{This indicates an 'alignment' process of the large 
models when processing information.}
\fixshu{What do you mean..?}

With growing utility of the large models especially as a 
mechanism for knowledge/information comprehension, this 
phenomenon poses significant risks to the fairness and 
diversity of information dissemination.
We leave the specific details of this process to future research. 



\warn{Beginning from the third iteration, the sample seems 
to have reached a "local optimum", with fewer edits needed, and ultimately, the 
large language model significantly expanded the original details and altered the style.}
\fixshu{What is the best place for this text..?}



The core components of ~\OurMODEL{} include:
two autophagous ("self-consuming") loops involving both large models and humans. They are designed to analyze how the interactions and preferences between humans and generative artificial intelligence lead to the dominance of synthesized data in the selection of model training datasets and information dissemination.
We aim to offer a novel perspective on the impact of large models, particularly in their role as intermediaries in human societal information dissemination, and the potential hazards this entails.
\fixme{What is the best place for this text..?}

\input{tables/distributionresult}

\section{Add to Results}
\begin{enumerate}
    \item In addition, to eliminate potential biases from lengthy contexts and granular scoring criteria, we set up a real-world scenario simulation. This tendency was also observed in results from crowd-sourced annotations.
    \item As well as the exacerbation of bias, which implies that the increasingly common use of model-generated data to train models~\ref{yu2023large} 
    induces a move towards local optima in model performance.

    \item We demonstrate that this will ultimately lead to the loss of 
    diversity in the model training data and human societal datasets, 
    as well as the exacerbation of bias.

    \item We illustrate this by verifying the biases of humans and large models as generators and disseminates of information when synthesizing and filtering information.

    \item This experiment demonstrated that, compared to authentic human data,

    \item Furthermore, \OurMODEL{} also demonstrates the risks associated with the deeper integration of large models extend beyond the methodologies 
    used in model training. 
    
    \item how the interactions and preferences between humans and generative artificial intelligence lead to the dominance of synthesized data in the selection of model training datasets and information dissemination.
    
    \item These loops emphasize the fact that the interaction process between AI systems and humans will lead the AI-generated data \warn{(aka synthetic data)} more likely to 
    win in messaging compared to real human data. 
    This causes a growing prevalence of \warn{AI-generated} synthetic data within within human society as well as model training datasets.

    \item This leads to the local optimum, where real human data increasingly struggles to enter model training and information exchange.
    
    \item There is a clear preference for synthetic data, 
    ultimately leading to a diminishing proportion of humanly 
    generated real data in the information cycle.

    \item Firstly, the core proposition of our reality model is that 
    large models and humans cannot maintain objectivity and 
    impartiality as part of the information dissemination loop.
    Furthermore, there is a clear preference for synthetic data, 
    ultimately leading to a diminishing proportion of human real 
    data in the information cycle.

    \item To demonstrate the inhibitory and promotive phenomena of 
    information transmission within Autophagous loops (as 
    indicated by the colored segments in Figure~\ref{fig:frameworklms} 
    and Figure~\ref{fig:framework_human}), 
    \warn{with dotted-red 
    representing inhibition and green representing facilitation.}

    \item 
\end{enumerate}




%%%%%%%%%%%%%%% EXTRA TEXT %%%%%%%%%%%%%%%


\eat{{\bf (i) metric-1.}
\warn{Cross-Scoring means every LLMs as scorer and generator at the same time.}
SHU: Both, they eva their own answer and others answer. Our experiments verify whether the model is an objective scorer and whether they give higher scores to themselves or their family models
They generate the answer with instructions in Table~\ref{table:prompt template Originally Generated Answer},~\ref{table:prompt template best Answer},~\ref{table:prompt template worst Answer}. And they evaluate their their own answer and other models answer with the metrics in table \ref{table:The prompt template for evaluating answers} 
{\bf (ii) metric-2.}}



\eat{As large models become increasingly important in information}

\eat{Specifically, Figure~\ref{fig:average_simchange} shows that after processing text using LLMs, the similarity between texts significantly increases, with the lower similarity tail being 'washed out', and the cross-similarity between sentences being enhanced.} 

\eat{What is motivation for 
Figure~\ref{fig:average_distributionchange}
especially wrt real vs LLM-generated data.} 


 
\eat{difference of the text relative to the previous}


\eat{The detailed explanation about the mathematical notation 
in Equation~\ref{Eq:data} is provided in Appendix~\ref{appendix:Dataset}
\eat{Appendix~\ref{appendix:Dataset} provides explanations of the corresponding mathematical notation, showing more details about the distribution of the dataset.}
\warn{For AI-washing experiment in text (Section~\ref{experiment：AI Washing}))}\warn{The raw text dataset construction process begins with the selection of passages from classic literature known for their rich stylistic features and thematic significance, where the English dataset is excerpted from the pile books3~\citep{pile}, and the Chinese passages are selected from WebNovel. A meticulous anonymization process is employed to prevent the large language model from identifying the textual sources. This involves the alteration of recognizable names, places, and events.}
\fixshu{ADD Explanation Why all of a sudden re-started explaining data..? This text needs to be moved. What is the relation between this and the explanation in the former para.}
The image dataset was constructed by \eat{carefully }selecting a 
subset of images from the \eat{comprehensive }ILSVRC data~\citep{ILSVRC15}
and web resources.
\eat{as well as other web image data, with selected} 
We select categories covering a wide range of topics and scenarios, 
in order to cover a broad range of visual features and complexity.
On the visual dataset, we sampled and cleaned the ILSVRC \citep{ILSVRC15} to ensure the diversity of image clarity and classification.}


\eat{For evaluation, we manually curated text and image data sets. 
For this, we initially handpicked 100 diverse question-answer 
pairs from Stack-Overflow and Quora as the seeds.
Subsequently, for each question in these pair, 
we used large models to generate initial responses 
with instruction in 
Table~\ref{table:prompt template Originally Generated Answer}.
We manually screened the most answered questions in 
Stack-Overflow and Quora, including psychology, books, 
mathematics, physics, and other fields.  At the same time, 
we selected fragments from the novel corpus for anonymization 
processing to study the behavior of the language model when 
delivering real human-generated data.
These responses were further processed to curate datasets 
rated as either 1 (lowest) or 5 (highest) in terms of quality,
similar to the self-alignment approach proposed by
~\citet{li2023selfalignment}.  
The prompts used for generating these diverse responses 
are detailed in Appendix \ref{appendix:Generation_Prompt_Template}. 
Final data set encompasses approximately 1,900 question-answer pairs. 
Formally, the dataset consists of a series of 22 tuples, each 
structured as follows:}
\eat{
\begin{equation}
\begin{aligned}
    T_j = \{d, Q, D, A\} \cup \bigcup_{i=0}^{5} \{A_{\text{model}_i}, \\ A_{\text{model}_i\text{score5}}, A_{\text{model}_i\text{score1}}\}
\end{aligned}
\end{equation}
\begin{equation}
\label{Eq:data}
    T_j = \{d, Q, D, A\} \cup \bigcup_{i=0}^{5} \{A_{\text{m}_i}, A_{\text{m}_i\text{s}_5}, A_{\text{m}_i\text{s}_1}\}
\end{equation}}

==> 5_limitations.tex <==
\section{Limitations} 
\noindent {\bf Selection of Models.} 
While we have experimented with LLMs that are available, many outstanding models are worth exploring in the future. These include the GLM family of models \citep{du-etal-2022-glm}, which are known for their innovative architectures, and the MoE-structured Mixtral 8x7B\footnote{\url{https://mistral.ai/news/mixtral-of-experts/}}, etc. In addition, some open-source multilingual models are also worth investigating, such as the Qwen series of models trained on a large Chinese corpus \citep{qwen} and the Arabic model Jais\footnote{\url{https://inceptioniai.org/jais/}}. Models with different languages, parameter sizes, and architectures exhibit different behaviors. In the field of visual models, more open-source and commercial models are worth investigating, such as Midjourney and DALL-E 3. In future research, we aim to deeply analyze the roles and characteristics of these models as an important part of human social information transfer.

\noindent {\bf Reliability of crowd-source Annotators.} 
A significant portion of our conclusions is derived from crowd-sourced annotators, sponsored by a start-up company's data annotation department. Of these annotators, 64 \% hold graduate degrees in science and engineering, and all possess proficient bilingual reading skills in Chinese and English. However, ensuring that their existing AI knowledge does not bias their judgments remains challenging. Additionally, the distribution of our annotators in the real world varies from the general user base of generative models. There is also an ongoing debate about the reliability of crowd-sourced workers\citep{9660043,TARASOV20146190}.  \citet{veselovsky2023artificial} have discussed the behavior of annotators using LLMs for labeling, which could compromise the reliability of the results.

==> XXTRA_experimentsbckup.tex <==
\section{Experimentation}
\label{sec:Experimentation}
In this section, we perform comprehensive experimentation
to evaluate the preferences of humans and language 
models in information selection. 
This helps us analyze how real human-generated data 
is suppressed in the human vs language model 
information dissemination loop.

The core evaluation objective is to:
(i) examine the preferences of both humans and LLMs in 
evaluation and filtration of information as part of the 
dissemination process;
(ii) investigated the potential drawbacks associated 
with using generative models for enhancing and transferring 
information.

\subsection{Experimental Settings}
\label{sec:exp-settings}
\noindent {\bf Datasets.}
For experimental evaluation, we curated three different sets of 
data sets, namely:
(i) QA-pairs,
(ii) Book3,
(iii) image-ax.
QA-pairs is a structured text data set used for: cross-scoring and 
mock-exam scenarios.
Book3 and image-ax are unstructured data sets used for AI-washing 
experiments for text and images respectively.
Detailed description and statistics of the data set is provided in
Appendix~\ref{appendix:Dataset}.





\noindent {\bf Large Models.}
We employed six different LLMs with varying architectures.
\eat{to generate and evaluate responses based on specific set of instructions} 
These include 
ChatGPT~\citep{li-etal-2022-gpt}, 
GPT-4~\citep{openai2023gpt4}, Claud2\footnote{\url{https://www.anthropic.com/index/claude-2}}, 
Llama-2-70b-chat~\citep{touvron2023llama}, 
PaLM2 chat-bison\footnote{\url{https://blog.google/technology/ai/google-palm-2-ai-large-language-model/}}, and 
Solar-0-70b-16bit\footnote{\url{https://huggingface.co/upstage/SOLAR-0-70b-16bit}}. 
We opted for relatively large-scaled models owing to their 
superior capabilities in instruction adherence, which we found 
lacking in small-scale models.
\eat{The focus on larger models in our experiments is due to their 
superior capability in instruction adherence and context length 
handling, which we found lacking in smaller-scale models.\fixme{Move it.}}
In assessing textual diversity, we used the models 
bge-large-zh-v1.5 and bge-large-en-v1.5
by~\citet{bge_embedding} as the embedding models.
For computer vision tasks, we utilized the open-source model 
StableDiffusionXL~\citep{podell2023sdxl}.

\noindent {\bf Evaluation Metrics.}
For cross-scoring experiments, we alternatively use LLMs as
response generators and evaluators. 
Corresponding template for using LLM as evaluator is shown in 
Table~\ref{table:The prompt template for evaluating answers} 
(Appendix~\ref{appendix:Cross_scoring_Prompt}).
This scoring criteria aims to verify the objective nature of LLMs 
as evaluators, i.e., whether a model assigns a higher 
scores to their response or response generated by other 
models.
For AI-washing experiments, we measure the diversity in information
after multiple rounds of iterations.
Specifically, for the text data, we cosine 
similarity (shown in Appendix~\ref{Appendix:datavec-sim}) 
to measure the diversity in original text and text 
reproduced by LLMs. 
For image data set, we visually analyze which features 
are preserved, omitted, and transformed by the LLMs.





\noindent {\bf Experimental Setup.}
\warn{Details about hyper-parameters + additional experimental settings..!}
For AI-washing value of N for text and images is \warn{XX} and \warn{YY} 
respectively.  
\fixshu{Fill experimental details here....!}


\subsection{Experimental Results}

\eat{Based on our discussion in Section \ref{sec:rat_risk}, i}


\eat{
For this, we designed three distinct experiments with details 
as follows:}
%\subsection{Experimental Setup}
%\label{Experimental Setup}
%\paragraph{\textbf{Datasets}}
\eat{For evaluation, we manually curated text and image data sets. 
For this, we initially handpicked 100 diverse question-answer 
pairs from Stack-Overflow and Quora as the seeds.
Subsequently, for each question in these pair, 
we used large models to generate initial responses 
with instruction in 
Table~\ref{table:prompt template Originally Generated Answer}. 
We manually screened the most answered questions in 
Stack-Overflow and Quora, including psychology, books, 
mathematics, physics, and other fields.  At the same time, 
we selected fragments from the novel corpus for anonymization 
processing to study the behavior of the language model when 
delivering real human-generated data.
These responses were further processed to curate datasets 
rated as either 1 (lowest) or 5 (highest) in terms of quality,
similar to the self-alignment approach proposed by
~\citet{li2023selfalignment}.  
The prompts used for generating these diverse responses 
are detailed in Appendix \ref{appendix:Generation_Prompt_Template}. 
Final data set encompasses approximately 1,900 question-answer pairs. 
Formally, the dataset consists of a series of 22 tuples, each 
structured as follows:}
\eat{
\begin{equation}
\begin{aligned}
    T_j = \{d, Q, D, A\} \cup \bigcup_{i=0}^{5} \{A_{\text{model}_i}, \\ A_{\text{model}_i\text{score5}}, A_{\text{model}_i\text{score1}}\}
\end{aligned}
\end{equation}
\begin{equation}
\label{Eq:data}
    T_j = \{d, Q, D, A\} \cup \bigcup_{i=0}^{5} \{A_{\text{m}_i}, A_{\text{m}_i\text{s}_5}, A_{\text{m}_i\text{s}_1}\}
\end{equation}}
\eat{The detailed explanation about the mathematical notation 
in Equation~\ref{Eq:data} is provided in Appendix~\ref{appendix:Dataset}
\eat{Appendix~\ref{appendix:Dataset} provides explanations of the corresponding mathematical notation, showing more details about the distribution of the dataset.}
\warn{For AI-washing experiment in text (Section~\ref{experiment：AI Washing}))}\warn{The raw text dataset construction process begins with the selection of passages from classic literature known for their rich stylistic features and thematic significance, where the English dataset is excerpted from the pile books3~\citep{pile}, and the Chinese passages are selected from WebNovel. A meticulous anonymization process is employed to prevent the large language model from identifying the textual sources. This involves the alteration of recognizable names, places, and events.}
\fixshu{ADD Explanation Why all of a sudden re-started explaining data..? This text needs to be moved. What is the relation between this and the explanation in the former para.}
The image dataset was constructed by \eat{carefully }selecting a 
subset of images from the \eat{comprehensive }ILSVRC data~\citep{ILSVRC15}
and web resources.
as well as other web image data, with selected 
We select categories covering a wide range of topics and scenarios, 
in order to cover a broad range of visual features and complexity.
On the visual dataset, we sampled and cleaned the ILSVRC \citep{ILSVRC15} 
to ensure the diversity of image clarity and classification.}

\input{tables/llm_prefer}

 







\noindent {\bf Cross-scoring Experiment.}
\label{sec:cross_scoring} 
To demonstrate the inhibitory and promotive phenomenon of information 
transmission within autophagous loops, we design cross-scoring 
experiments using QA-pairs data set.


We focus on whether LLMs and humans remain impartial while 
filtering and transmitting information, and, if not, what 
kind of bias they induce.

We prompt each model to assess not only the answers generated by 
other models but also those produced by humans. The scoring 
range is between 1 to 5 (see 
Table~\ref{table:The prompt template for evaluating answers}). 
%\fixshu{Though understandable, yet this sentence is confusing}
For instance, in the \warn{"five-score answers" segment,see Table~\ref{table:The prompt template for evaluating answers}}, an 
answer generated by ChatGPT would be evaluated by other LLMs like 
GPT4 and Claud2, assigning a score within the 1-5 range based on 
its quality. 
\fixshu{IT MEANS the score from 1 to 5 what is five-score answer segment..?}

At the same time, we employed fifty crowd-sourced annotators 
to rate all question-answer pairs, based on the 
scoring criteria in 
Table~\ref{table:Scoring criteria for crowdsourced annotations}. 
\fixshu{Fixed what do you mean by: rate all question-answer pairs equally? }

We recorded the average scores for all samples, excluding 
instances where the models refused to respond.


% {Comparative Analysis of Human and AI Performance in Information Screening and Filtering}
\noindent {\bf Exam Scenario Simulation.}
\label{sec:exam scenario}
\fixshu{Fixed Explain what is filtering + screening..?}
\warn{The large model filters out the preferred data and filters out other data by a certain evaluation metric, which is shown in detail in our experiments:Table \ref{table:The prompt template for evaluating answers} and Figure \ref{fig:Exam_Scenario_Simulation} }

In this experiment, we present our experimental design to 
answer the following question: Human-generated or AI-generated 
answers, which one wins in information screening and filtering? 
% \input{tables/human_AND_llm}

Its process-flow is explained in 
Figure~\ref{fig:Exam_Scenario_Simulation}, 
which illustrates the examination scenario where answers 
generated by LLMs (e.g., ChatGPT and Claud2,) alongside 
those produced by humans, were anonymized to mitigate any bias. 

To further eliminate the potential influence of the sequence 
in which the answers were presented, we randomized their order.

Both language models and human participants, assuming the role 
of experts, were then asked to assign scores to these 
answers on a percentile scale, and choosing the best answer.
\fixshu{IT means score from 0-100 . what is percentile scale.? }

\noindent {\bf AI-washing.} 
\label{experiment：AI Washing}
For AI-washing experiments, we analyze the abilities of large models 
as faithful messengers of information?
Basically, we aim to answer the following questions:

(i) do these models capture the main points in the information that 
needs to be conveyed? 

(ii) whether large models play the role of a link in the information 
transmission that may also lead to losses.
\eat{whether large models play the role of an important 
link in the transmission of information can lead to important losses.}

We instruct SDXL~\citep{podell2023sdxl} and ChatGPT\footnote{\url{https://openai.com/blog/chatgpt}} to process these samples $N$ times, 
respectively. 
\fixshu{FIxed Add Citation for SDXL and chatGPT}
The prompts used for these experiments are provided 
in Table~\ref{table:aiwashprompt}. 

\subsection{Analyses}

\subsubsection{Information Selection Biases\eat{ in Human and Language Model Interactions}}

\noindent {\bf LLMs can identify the quality of response as 
information filters but are obviously biased towards synthetic data.
\warn{Or biased towards synthetic data}\fixshu{FIXED check it}} 

Table~\ref{table:exp1} displays the cross-scoring results for various 
LLMs on a five-point scale. 
These results \eat{from this evaluation allow help us discern:}
help us understand that
LLMs do have an inherent capability to comprehend 
\eat{grading standards} \warn{specific criteria} \fixshu{FIXED it means criteria we prompt them to follow the What are the grading standards..?} 
and can adjust the quality of their generated answers based 
on relevant instructions. 

However, when scoring data according to these 
criteria, each model exhibits certain preferences.
\fixshu{It means the criteria we prompt LLM to follow 文、hen scoring ;Which criteria}

Specifically, models tend to assign higher scores to the high-quality 
answers generated by themselves, particularly for ChatGPT and GPT-4, 
which both demonstrate high confidence in their own outputs. 
Also, we find that 
ChatGPT and GPT-4 exhibit similar characteristics in scoring; 
they are inclined to extreme scores, i.e., high or low scores 
(assigning scores of 1 or 5 with very high probability), 
at the same time, they both tend to 
assign lower scores to Claude2 and PaLM 2 chat-bison.
These results are aligned with earlier research by~
\citet{liu2023llms} that emphasized that current 
top-performing LLMs (both black-box and white-box)
are narcissistic evaluators.\fixme{Move text to concluding results}


While evaluating the abilities of LLMs as 
\warn{answer generators\eat{of answers}}, ChatGPT’s worst 
quality answers can still deceptively obtain higher scores 
from other models, that are easy to figure out for humans 
via crowd-sourcing.
\eat{ workers can tell them.} 
\eat{At the same time, as the generator of answers, ChatGPT’s worst quality 
answers can still deceptively obtain higher scores from other models, 
but human crowd-sourcing workers can tell them.}
Furthermore, we observed that Claud2 tends to favor neutral 
and 'less controversial' ratings, often 
assigning average scores, i.e., 3 or 4, even for the worst quality answers. 
This is also reflected by a relatively higher score assigned 
by Claud2 to low-quality answers compared to other models. 
\eat{is much higher than that of other models,} 
Also, the difference between its score for initial answers and 
best-quality answers is not significant.


Llama-2-70b-chat and Solar-0-70B-16bit show similar scoring and generation behaviors, which may be attributable to the fact
that \warn{Solar-0-70B-16bit is fine-tuned form LLaMA-2-70b with only Orca-style and 
Alpaca-style dataset,
\fixshu{FIXED fine-tuned using LLAma-2-70B instructions..?}
indicating that the pre-trained model has a significant influence on the model's preferences.}

We observed that prompting the model to generate better answers did 
not always lead to higher scores in our experiments. Only Claud2 
showed significant improvement in the answers compared to the 
original responses. 
\warn{Conversely, when the model generated poorer answers, the overall 
effect was notably significant.}
\fixshu{Re-write this line is not clear..!}

However, ChatGPT and Palm-2-chat-bision still achieved relatively high scores, a possible reason is could be attributed to the models being highly aligned to avoid producing harmful outputs~\citep{lambert2022illustrating}. 
\fixshu{How this alignment helps in achieving higher score..?}
We leave further investigation to our future work.
\fixshu{For this part, the heading says:\\
\textbf{LLMs can identify the quality of response as
information filters but are obviously biased
against real human data.} 
I think The true message is not conveyed as there is hardly any
discussion on real human data..????}

\warn{These facts remind us more cost-effective model training processes and wider applications are inevitable trends of large model development, so we need to discuss not only the technology of large models themselves but also the roles they play in their iterations and the development of human society \citep{tomavsev2020ai}.}\fixme{Asif move text}

\noindent {\bf Human-generated answers receive lower scores.} 
In Table \ref{table:exp1}, 
\fixshu{which part of Table~\ref{table:exp1}..?}
we observe that human-generated responses received relatively 
lower scores from the LLMs. 

Upon analysis, we found that human evaluators were able to objectively assess the answers produced by the LLMs, demonstrated by the fact that their scores for high-quality answers consistently remained above 4.00 when confronted with the results generated by the large language model, while the results for lower-quality answers remained below 3.00. 
\fixshu{Cut down the above sentence into two meaningful sentences.}

Furthermore, the scoring behavior of \eat{our 50 }crowd-sourced annotators toward the answers generated by the large language model was largely consistent. This may be due to the highly structured and standardized nature of answers produced by AI systems aligned with human feedback\eat{, which often received higher scores}. 
\warn{In contrast, human-generated answers received lower scores 
from the \fixshu{human..?} annotators, with significant variations 
among different evaluators. 
This may be attributed to the higher alignment degree between 
the large model and the human collective, compared to the 
alignment among individual humans.}
\fixshu{You mean humans are more aligned with LLMs,
compared to alignment between humans only.?}


\subsubsection{LLMs-generated Answers are more likely to Win in Information Screening}
\input{tables/human_round} 
To mitigate the impact of scoring criteria
\fixshu{what do yo mean by scoring criteria}
and excessive context length
\fixshu{why we need to mention excessive context length.?}
on the evaluative capabilities of large models and 
human evaluators, we simulated an examination grading scenario. 

For this, we used LLMs (ChatGPT, Claud2) and humans to simultaneously act as generator and evaluators.
The results for this experiment (Table \ref{table:Exam_Scenario_Simulation})
show that that human answers were \warn{rarely} chosen as 
the best response, indicating a challenge in integrating authentic human-generated responses into the training data for models and the real-world human feedback loop.
\fixshu{say little more based on Table~\ref{table:Exam_Scenario_Simulation}.}
This finding substantiates the potential risks highlighted in Section \ref{sec:rat_risk} that
emphasized that human-generated responses receive comparatively lower scores.
\fixme{Asif: Correlate with Sec~\ref{sec:rat_risk}.}


\eat{Furthermore, we engaged ChatGPT, Claud2, and crowd annotators to select the best answers.}



\subsubsection{\eat{LLMs as Biased }Information Transmitters}
\input{tables/SDXL_0}
\input{tables/aiwashresult_img}
\eat{\noindent {\bf Large models exhibit inherent biases regarding the manner and content of conveyed information.}}

\noindent {\bf Large models are inherently biased.}
We claim that the large models are inherently biased 
regarding the manner and content of conveyed information.

\warn{For this, we...!\\
Where details + specs for AI-Washing experiments}.?

An example in this regard is illustrated in 
Table~\ref{table:aiwashtext}, where we show the 
results of a sample text data being refined simultaneously by ChatGPT five times.
We observe the refinements induced subtle shifts 
in the sample's language style and narrative technique.


We also repeat these experiments for the image data 
sets. For this, we used \textbf{\warn{XX}}\fixshu{add details} model to refine a set of images for 20 rounds. 
Corresponding results for a vast variety of images 
are shown in Figure~\ref{fig:SDXL_0.png} and \ref{fig:aiwashimag}.
These results \eat{show Our observations }reveal that repeatedly processing images with generative models is akin to information and feature filtration process. 
The model decides which specific aspects to preserve, diminish, or amplify based on its inherent \warn{biases.}
\fixshu{which biases.?}

Specifically, in Figure \ref{fig:SDXL_0.png}, the 
model preserved the color distribution of the original
image but altered the main subject from a cat to a 
human portrait. 
Conversely, for the images in Figure~\ref{fig:aiwashimag}, 
we observed, a dominant alteration in image style rather than a change in the primary content for first, forth and fifth images.
Whereas, the images at second and third position underwent several iterations with minimal transformation, with the 
third image lost readability for the textual content.


This inconsistency may be attributed to the fact that while SDXL is renowned for generating high-quality images, the definition of quality in the context of generative models is subjective and heavily influenced by the annotations of the training dataset, also explained in detail by~\citet{podell2023sdxl}. 

These observations also indicate a bias in the model's processing, where certain features are selectively preserved or altered based on the model's training objective and inherent design. 
This in turn results in a higher probability of generating images containing specific features and/or information, e.g.,
loop, such as hand-drawn styles, portraits, close-ups of objects with clear backgrounds, etc.
To summarize, these findings demonstrate that large models are inherently biased regarding the manner and content of conveyed information.
\input{tables/embedding0-4}


\noindent {\bf \eat{The risk to the fairness and }
Diversity of information spread.}

In order to further understand the training behaviour of large
models, we analyzed the cosine similarity scores during model 
training for humanly-generated and LLM-generated text.

\warn{The results in Figure~\ref{fig:average_simchange} shows that after processing text using LLMs, the similarity between texts significantly increases, with the lower similarity tail being 'washed out', and the cross-similarity between sentences being enhanced.}
\fixshu{Re-write to make it explicit.}
\warn{This shows that \eat{We observe that }while acting as 
information disseminators, the large models exhibit some 
unique characteristics, i.e.,\eat{Their optimization objective} 
they tends to optimize more for real-world data while being 
more lenient towards self-generated samples.}
\eat{
To validate these findings, we perform a simple 
For this Experiments demonstrate that when}

\input{tables/average_distributionchange}
% \input{tables/distributionresult}


Analyzing the model behavior across multiple runs, 
we can see that after approximately three iterations 
($N\approx3$), the difference in the average 
cosine similarity across multiple runs round tends 
to stabilize (Figure~\ref{fig:average_distributionchange}).
\warn{This indicates an 'alignment' process of the large 
models when processing information.}
\fixshu{What do you mean..?}

With growing utility of the large models especially as a 
mechanism for knowledge/information comprehension, this 
phenomenon poses significant risks to the fairness and 
diversity of information dissemination.
We leave the specific details of this process to future research. 



\warn{Beginning from the third iteration, the sample seems 
to have reached a "local optimum", with fewer edits needed, and ultimately, the large language model significantly expanded the original details and altered the style.}
\fixshu{What is the best place for this text..?}



The core components of ~\OurMODEL{} include:
two autophagous ("self-consuming") loops involving both large models and humans. They are designed to analyze how the interactions and preferences between humans and generative artificial intelligence lead to the dominance of synthesized data in the selection of model training datasets and information dissemination.
We aim to offer a novel perspective on the impact of large models, particularly in their role as intermediaries in human societal information dissemination, and the potential hazards this entails.
\fixme{What is the best place for this text..?}



\section{Add to Results}
\begin{enumerate}
    \item In addition, to eliminate potential biases from lengthy contexts and granular scoring criteria, we set up a real-world scenario simulation. This tendency was also observed in results from crowd-sourced annotations.
    \item As well as the exacerbation of bias, which implies that the increasingly common use of model-generated data to train models~\ref{yu2023large} 
    induces a move towards local optima in model performance.

    \item We demonstrate that this will ultimately lead to the loss of 
    diversity in the model training data and human societal datasets, 
    as well as the exacerbation of bias.

    \item We illustrate this by verifying the biases of humans and large models as generators and disseminates of information when synthesizing and filtering information.

    \item This experiment demonstrated that, compared to authentic human data,

    \item Furthermore, \OurMODEL{} also demonstrates the risks associated with the deeper integration of large models extend beyond the methodologies 
    used in model training. 
    
    \item how the interactions and preferences between humans and generative artificial intelligence lead to the dominance of synthesized data in the selection of model training datasets and information dissemination.
    
    \item These loops emphasize the fact that the interaction process between AI systems and humans will lead the AI-generated data \warn{(aka synthetic data)} more likely to 
    win in messaging compared to real human data. 
    This causes a growing prevalence of \warn{AI-generated} synthetic data within within human society as well as model training datasets.

    \item This leads to the local optimum, where real human data increasingly struggles to enter model training and information exchange.
    
    \item There is a clear preference for synthetic data, 
    ultimately leading to a diminishing proportion of humanly 
    generated real data in the information cycle.

    \item Firstly, the core proposition of our reality model is that 
    large models and humans cannot maintain objectivity and 
    impartiality as part of the information dissemination loop.
    Furthermore, there is a clear preference for synthetic data, 
    ultimately leading to a diminishing proportion of human real 
    data in the information cycle.

    \item To demonstrate the inhibitory and promotive phenomena of 
    information transmission within Autophagous loops (as 
    indicated by the colored segments in Figure~\ref{fig:frameworklms} 
    and Figure~\ref{fig:framework_human}), 
    \warn{with dotted-red 
    representing inhibition and green representing facilitation.}

    \item 
\end{enumerate}




%%%%%%%%%%%%%%% EXTRA TEXT %%%%%%%%%%%%%%%


\eat{{\bf (i) metric-1.}
\warn{Cross-Scoring means every LLMs as scorer and generator at the same time.}
SHU: Both, they eva their own answer and others answer. Our experiments verify whether the model is an objective scorer and whether they give higher scores to themselves or their family models
They generate the answer with instructions in Table~\ref{table:prompt template Originally Generated Answer},~\ref{table:prompt template best Answer},~\ref{table:prompt template worst Answer}. And they evaluate their their own answer and other models answer with the metrics in table \ref{table:The prompt template for evaluating answers} 
{\bf (ii) metric-2.}}



\eat{As large models become increasingly important in information}

\eat{Specifically, Figure~\ref{fig:average_simchange} shows that after processing text using LLMs, the similarity between texts significantly increases, with the lower similarity tail being 'washed out', and the cross-similarity between sentences being enhanced.} 

\eat{What is motivation for 
Figure~\ref{fig:average_distributionchange}
especially wrt real vs LLM-generated data.} 


 
\eat{difference of the text relative to the previous}


\eat{The detailed explanation about the mathematical notation 
in Equation~\ref{Eq:data} is provided in Appendix~\ref{appendix:Dataset}
\eat{Appendix~\ref{appendix:Dataset} provides explanations of the corresponding mathematical notation, showing more details about the distribution of the dataset.}
\warn{For AI-washing experiment in text (Section~\ref{experiment：AI Washing}))}\warn{The raw text dataset construction process begins with the selection of passages from classic literature known for their rich stylistic features and thematic significance, where the English dataset is excerpted from the pile books3~\citep{pile}, and the Chinese passages are selected from WebNovel. A meticulous anonymization process is employed to prevent the large language model from identifying the textual sources. This involves the alteration of recognizable names, places, and events.}
\fixshu{ADD Explanation Why all of a sudden re-started explaining data..? This text needs to be moved. What is the relation between this and the explanation in the former para.}
The image dataset was constructed by \eat{carefully }selecting a 
subset of images from the \eat{comprehensive }ILSVRC data~\citep{ILSVRC15}
and web resources.
\eat{as well as other web image data, with selected} 
We select categories covering a wide range of topics and scenarios, 
in order to cover a broad range of visual features and complexity.
On the visual dataset, we sampled and cleaned the ILSVRC \citep{ILSVRC15} to ensure the diversity of image clarity and classification.}


\eat{For evaluation, we manually curated text and image data sets. 
For this, we initially handpicked 100 diverse question-answer 
pairs from Stack-Overflow and Quora as the seeds.
Subsequently, for each question in these pair, 
we used large models to generate initial responses 
with instruction in 
Table~\ref{table:prompt template Originally Generated Answer}.
We manually screened the most answered questions in 
Stack-Overflow and Quora, including psychology, books, 
mathematics, physics, and other fields.  At the same time, 
we selected fragments from the novel corpus for anonymization 
processing to study the behavior of the language model when 
delivering real human-generated data.
These responses were further processed to curate datasets 
rated as either 1 (lowest) or 5 (highest) in terms of quality,
similar to the self-alignment approach proposed by
~\citet{li2023selfalignment}.  
The prompts used for generating these diverse responses 
are detailed in Appendix \ref{appendix:Generation_Prompt_Template}. 
Final data set encompasses approximately 1,900 question-answer pairs. 
Formally, the dataset consists of a series of 22 tuples, each 
structured as follows:}
\eat{
\begin{equation}
\begin{aligned}
    T_j = \{d, Q, D, A\} \cup \bigcup_{i=0}^{5} \{A_{\text{model}_i}, \\ A_{\text{model}_i\text{score5}}, A_{\text{model}_i\text{score1}}\}
\end{aligned}
\end{equation}
\begin{equation}
\label{Eq:data}
    T_j = \{d, Q, D, A\} \cup \bigcup_{i=0}^{5} \{A_{\text{m}_i}, A_{\text{m}_i\text{s}_5}, A_{\text{m}_i\text{s}_1}\}
\end{equation}}

==> figures/self-alignmentresult.tex <==
\begin{table*}[!ht]
    \centering
    \begin{tabular}{llllll}
    \hline
        Model & Average & ARC & HellaSwag & MMLU & TruthfulQA \\ \hline
        Llama-2-7b & 54.32 & 53.07 & 78.59 & 46.87 & 38.76 \\ 
        Llama-2-7b-chat & 56.34 & 52.90 & 78.55 & 48.32 & 45.57 \\ 
        Vicuna-7b-v1.3 & 55.62 & 50.43 & 76.92 & 48.14 & 47.01 \\ 
        Humback 0 & 57.43 & 55.47 & 80.45 & 46.73 & 44.67 \\ 
        Humback 1 & 55.99 & 52.99 & 73.24 & 46.44 & 40.03 \\ 
        Humback 2 & 54.29 & 52.31 & 71.83 & 46.07 & 39.92 \\ \hline
    \end{tabular}
\end{table*}

\begin{table*}[!ht]
    \centering
    \begin{tabular}{lllll}
    \hline
        Model & win\_rate & Standard\_error & n\_total & avg\_length \\ \hline
        gpt 4 & 73.79 & 1.54 & 805 & 1365 \\ 
        claude & 70.37 & 1.60 & 805 & 1082 \\ 
        chatgpt & 66.09 & 1.66 & 805 & 811 \\ 
        vicuna-13 b & 64.10 & 1.69 & 805 & 985 \\ 
        falcon-40 b-instruct & 56.52 & 1.74 & 805 & 1037 \\ 
        text\_davinci\_003 & 50.00 & 0.00 & 805 & 662 \\ 
        alpaca-7 b & 45.22 & 1.74 & 805 & 307 \\ 
        Humback 0 & 37.43 & 1.68 & 805 & 572 \\ 
        text\_davinci\_001 & 28.07 & 1.56 & 805 & 296 \\ 
        Humback 1 & 25.90 & 1.44 & 805 & 1560 \\ 
        Humback 2 & 27.49 & 1.59 & 805 & 1610 \\ \hline
    \end{tabular}
\end{table*}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/aiwash.tex <==
\begin{table*}[!ht]
    \centering
    \caption{prompt}
    %  \begin{tabularx}{0.9\textwidth}{XXX} % 
    \begin{tabularx}{0.9\textwidth}{>{\hsize=.3\hsize}X>{\hsize=.3\hsize}X>{\hsize=1.4\hsize}X} 
    \hline
    Sample Category & Model & Prompt \\ 
    \hline
    Text & ChatGPT & Polish the following paragraph:\{TEXT\} \\
    Image & SDXL & {Positive: best quality, masterpiece, best quality, extremely detailed; Negative: distortion, cutoff, low contrast, underexposed, overexposed, blur, draft, grainy}\\ 
    \hline
    \end{tabularx}
    \label{table:prompt}
\end{table*}

% \begin{table}[!ht]
%     \centering
%     \caption{prompt}
%     \small 
%     \begin{tabularx}{0.9\columnwidth}{|>{\hsize=.3\hsize}X|>{\hsize=.3\hsize}X|>{\hsize=1.4\hsize}X|} 
%     \hline
%     Sample Category & Model & Prompt \\ 
%     \hline
%     Text & ChatGPT & Polish the following paragraph:\{TEXT\}  \\
%     Image & SDXL & \makecell[l]{Positive: best quality, masterpiece, best quality, extremely detailed\\Negative: distortion, cutoff, low contrast, underexposed, overexposed, blur, draft, grainy}\\ 
%     \hline
%     \end{tabularx}
%     \label{table:prompt}
% \end{table}


==> tables/aiwashresult_img.tex <==
\begin{figure}[b]
\centering
\vspace{-3.7ex}
\includegraphics[width=0.85\textwidth]{figures/aiwashimg.pdf}
\vspace{-2.1ex}
\caption{After 20 rounds of AI-washing experiments with the SDXL model~\citep{podell2023sdxl}, 
it becomes evident that different images retain and discard details in 
varying manners. \eat{This suggests that generative models tend to emphasize 
or de-emphasize certain features, revealing their unique patterns of recognizing, understanding, and reconstructing visual content.}}
\label{fig:aiwashimag}
\end{figure}

==> tables/average_distributionchange.tex <==
\begin{figure}[b]
\centering
\includegraphics[width=0.4\textwidth]{figures/average_distributionchange.jpg}
\caption{The average cosine similarity difference over a series of 20 iterations.}
\vspace{-2.7ex}
\label{fig:average_distributionchange}
\end{figure}

==> tables/embedding0-4.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{figures/distribution_0-4.pdf}
\caption{Density distributions of cosine similarity 
scores for entities processed $N$ times by LLM.
\warn{Explain it in caption.}}
\vspace{-2.7ex}
\label{fig:average_simchange}
\end{figure}

==> tables/framework2.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=0.5\textwidth]{figures/frameworkhuman.pdf}
\caption{\textbf{Our testing HUMAN framework.} }
\label{fig:framework_human}
\end{figure*}

==> tables/round.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=0.8\textwidth]{figures/round.pdf}
\caption{\textbf{round} }
\label{fig:exp1}
\end{figure*}

==> tables/text.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=0.95\textwidth]{figures/text.png}
\caption{\textbf{Multiple processing of human-generated text using Large Language models and prompts that are only used to control the quality of the text still can lead to serious discrepancy loss and information bias.} As large language models are widely used for tasks such as text generation and text proofreading, synthetic data that has been embellished by LLMs is growing rapidly and is difficult to discern, and can easily be re-entered for model training and inference. We have designed experiments to demonstrate that by merely prompting the model to embellish and improve the quality of the input text, after many trials (in fact, in our case no more than six) the diversity of the text is severely lost and much important information is misrepresented (most of which is content that is unfamiliar to the LLMs themselves).}
\label{fig:text.png}
\end{figure*}
